Decoherence as detector of the Unruh effect, II

The Unruh effect remains a central topic in quantum field theory, although its direct experimental verification continues to be challenging. Recent efforts have therefore focused on indirect detection strategies in which the Unruh effect emerges through measurable physical processes. In this work, we extend a previously introduced detector model, originally formulated for a massless scalar field, to the electromagnetic field. We show that the decoherence decay rates differ between inertial and accelerated frames. Furthermore, we demonstrate that the characteristic exponential decay associated with the Unruh effect can be observed at lower accelerations than those considered in earlier studies.

==> SM.tex <==


